CityPlanner: A Sandbox Agent for Executable Urban Planning

Urban planning is a real-world spatial optimization problem that requires selecting feasible actions from large candidate spaces under practical objectives such as cost and service quality. Existing optimization and reinforcement learning methods are effective for fixed formulations, but often depend on task-specific representations and constraint handling. We propose \emph{CityPlanner}, a sandbox-agent framework for executable urban planning. CityPlanner introduces \emph{UrbanSandbox}, a unified file-based environment where agents inspect task files, generate plans, run evaluators, and revise decisions based on executable feedback. To make learning tractable, we further propose atomic-task reinforcement learning, which decomposes long sandbox trajectories into \emph{BuildPlan} for initial construction and \emph{ImprovePlan} for feedback-based refinement. Experiments on a real-world benchmark show that CityPlanner consistently outperforms heuristic, task-specific RL, and general LLM-agent baselines. Ablations verify the contributions of UrbanSandbox, atomic-task RL, and iterative deployment. We release the code and dataset at https://anonymous.4open.science/r/co-agent-C1C8

==> 1-intro-bp.tex <==
\section{Introduction}

Urban planning is a fundamental problem in city management. It converts spatial data, infrastructure conditions, and policy objectives into concrete decisions over land use, road construction, and public facilities~\citep{zheng2025urban,liu2025large,zheng2023road,von2022reinforcement,liu2023optimal}. These decisions have direct influence on transportation efficiency, service accessibility, energy infrastructure, ecological quality, and residents' living conditions. From an optimization perspective, urban planning is challenging because it involves large combinatorial action spaces, hard feasibility constraints, and multiple competing objectives, such as construction cost, spatial coverage, fairness, environmental benefit, and livability. Moreover, the effect of each planning action is highly context-dependent, since its value is determined by surrounding population, road topology, existing facilities, land functions, and local demand patterns.

\begin{figure}[tbp]
    \centering
    \includegraphics[width=\linewidth]{figures/demo.png}
    \caption{Illustration of executable urban planning with CityPlanner. The agent interacts with UrbanSandbox by reading task files, generating plans, running evaluators, and revising decisions based on executable feedback.}
    \label{fig:demo}
\end{figure}

A large body of work has studied urban planning with optimization, heuristic search, and reinforcement learning methods~\citep{rasheed2020deep,von2022reinforcement,zheng2023road}. These methods are effective when the problem structure is well specified and the state representation, action space, constraints, and objective function are fixed in advance. However, practical urban planning tasks are often heterogeneous. Different planning tasks may involve different candidate types, constraint definitions, evaluation procedures, and feedback forms. As a result, methods designed for one task or one representation usually require non-trivial redesign when transferred to another task. This limits their applicability as a unified planning interface across diverse urban scenarios.

Recent large language model agents provide a new possibility for handling such heterogeneous planning interfaces. Instead of being restricted to a predefined vectorized state-action representation, an LLM agent can read task descriptions, inspect structured files, write intermediate analyses, execute tools, and revise its solution according to feedback~\citep{yao2023react,shinn2023reflexion,qintoolllm,patilgorilla}. Nevertheless, directly using an LLM as a black-box planner is insufficient for constrained urban planning. A generated plan must satisfy explicit feasibility constraints and must be evaluated by task-specific programs rather than by natural-language plausibility. Therefore, the key question is not whether an LLM can directly output a final plan, but how to ground its reasoning process in an executable environment where plans can be verified, scored, and iteratively improved.



In this paper, we formulate urban planning as an executable sandbox-agent problem. For each planning instance, the agent is placed in a sandbox that contains city data, candidate actions, task constraints, executable evaluators, and output interfaces. The agent solves the task by interacting with the sandbox: it reads input files, constructs a plan, runs the evaluator, observes diagnostic feedback, and revises the plan when necessary. This formulation provides a common interaction protocol for heterogeneous urban planning tasks while preserving their task-specific objectives and constraints.

However, training an LLM agent in such a sandbox is non-trivial. Complete sandbox trajectories are long and noisy. A trajectory may contain repeated file inspection, script execution, invalid submissions, and intermediate revisions. As the interaction proceeds, outdated observations and failed attempts accumulate in the context, making the effective state increasingly difficult to use. In addition, the main planning reward is usually available only after a complete plan is submitted and evaluated. This creates a sparse-reward and long-horizon credit assignment problem: the model must learn which earlier decisions contributed to final feasibility and objective quality. Direct reinforcement learning over complete trajectories can therefore improve superficial behaviors such as output formatting or command execution, while still failing to produce high-quality plans.

To address these issues, we propose \emph{CityPlanner}, a sandbox-agent framework for executable urban planning. CityPlanner consists of two components. First, we introduce \emph{UrbanSandbox}, a unified file-based environment for land allocation, road construction, and EV charging station placement. Each instance provides visible city states, candidate actions, constraints, and an executable evaluator. The agent interacts with the environment through a minimal \texttt{bash}-based interface, which allows general file inspection, plan generation, script execution, and evaluator invocation without relying on task-specific agent APIs. Second, we propose \emph{atomic-task reinforcement learning}, which decomposes long-horizon sandbox planning into two finite-context tasks. \emph{BuildPlan} learns to construct an initial feasible plan from the task files, while \emph{ImprovePlan} learns to revise an existing plan using evaluator diagnostics. At inference time, CityPlanner composes these two tasks into an iterative procedure: it first builds an initial plan and then repeatedly evaluates, improves, and re-evaluates the best-so-far solution.
For empirical evaluation, we collect real-world data from OpenStreetMap~\cite{osm} and build an executable benchmark for urban planning, covering 5,670 planning instances over 1,890 urban tiles across three tasks. Experiments show that CityPlanner consistently improves planning quality over heuristic, task-specific RL, and LLM-agent baselines, while ablations confirm the contributions of UrbanSandbox, atomic-task RL, and iterative refinement.



% The main contributions of this paper are summarized as follows:
% \begin{itemize}[leftmargin=*]
%     \item We formulate executable urban planning as a sandbox-agent problem and instantiate it with UrbanSandbox, a unified file-based environment with task-specific constraints and evaluators.

%     \item We propose atomic-task reinforcement learning, which decomposes long-horizon sandbox interaction into BuildPlan and ImprovePlan for shorter contexts and clearer credit assignment.

%     \item We construct an OpenStreetMap-based executable benchmark and show that CityPlanner consistently outperforms baselines across tasks and difficulty levels.
% \end{itemize}



==> 3-method-bp.tex <==
\section{Problem Statement}
\label{subsec:problem}

Urban planning aims to improve an existing urban region by selecting planning actions under task-specific constraints. In this work, we consider three representative tasks: 

\noindent~$\bullet$ \emph{Land allocation} assigns land-use types to candidate parcels to improve functionality and livability under land-use, spatial, ecological, and service-balance constraints.

\noindent~$\bullet$ \emph{Road construction} selects road segments to add to the existing network to improve connectivity and mobility under budget, quantity, and spatial-validity constraints.


\noindent~$\bullet$ \emph{Station placement} selects candidate sites for new charging facilities to improve accessibility and coverage under demand, capacity, infrastructure, and cost constraints.

Although these tasks involve different spatial objectives, they share the same decision structure: given an urban region and a finite set of candidate actions, the planner selects a constraint-satisfying subset of candidates as the final plan.
Formally, we provide a unified definition for the three planning tasks. Each instance $p$ is represented by an attributed city graph
\begin{equation}
\mathcal{G}_p=(V_p,E_p,\mathbf{X}^V_p,\mathbf{X}^E_p),
\end{equation}
where $V_p$ denotes urban spatial units, such as parcels, facilities, or candidate sites, and $E_p$ denotes road-network edges. The matrices $\mathbf{X}^V_p$ and $\mathbf{X}^E_p$ encode node and edge attributes, respectively. Each instance provides a finite candidate set $\mathcal{C}_p\subseteq V_p\cup E_p$, where each candidate corresponds to a task-specific planning action. A plan $P\subseteq\mathcal{C}_p$ selects a subset of candidates as the final planning decision. We use an aggregate constraint function $\Psi_p(P,\mathcal{G}_p)\in\{0,1\}$ to indicate whether $P$ satisfies all task-specific constraints induced by the graph structure and attributes. The planning quality of $P$ is measured by a task-specific score $S_p(P)$. The goal is to find a feasible plan with the highest score:
\begin{equation}
P_p^\star
=
\arg\max_{P\subseteq\mathcal{C}_p:\Psi_p(P,\mathcal{G}_p)=1}
S_p(P).
\end{equation}
Detailed definitions are provided in Appendix~\ref{app:task_definitions}.



\section{Method}
\label{sec:method}
Urban planning tasks are challenging due to their large candidate spaces and spatially grounded constraints. As shown in Figure~\ref{fig:demo}, CityPlanner addresses this challenge with UrbanSandbox, a unified executable interface that allows the agent to inspect task files, generate plans, run evaluators, and receive constraint and score feedback. To make learning tractable, CityPlanner further decomposes long planning trajectories into two atomic tasks: BuildPlan for initial plan construction and ImprovePlan for feedback-based revision. At inference time, the two skills are composed iteratively to solve longer-horizon planning tasks within bounded contexts.

\subsection{UrbanSandbox}
\label{subsec:urbansandbox}

The problem statement defines the planning objective. UrbanSandbox specifies how each planning instance is exposed to an agent as an executable environment. For each instance $p$, we construct
\begin{equation}
\mathcal{E}_p =
\langle
\mathcal{I}_p,\mathcal{W}_p,\mathcal{O}_p,
\operatorname{Exec}_p,\operatorname{Eval}_p
\rangle .
\end{equation}
Here, $\mathcal{I}_p$ is the read-only input space, $\mathcal{W}_p$ is the writable workspace, $\mathcal{O}_p$ is the output space, $\operatorname{Exec}_p$ executes commands, and $\operatorname{Eval}_p$ evaluates plans.

UrbanSandbox is implemented as a file-based sandbox. The \texttt{input/} directory contains the visible city state, candidate set, task schema, constraints, and evaluator. The \texttt{work/} directory is used for intermediate analyses and scripts. The \texttt{outputs/} directory stores submitted plans and evaluation results. This interface keeps the task representation explicit and avoids task-specific agent APIs.

The agent interacts with UrbanSandbox through a minimal \texttt{bash}-based interface. At step $t$, the policy emits a shell command
\begin{equation}
a_t\sim\pi_\theta(\cdot\mid h_t),
\end{equation}
where $h_t=(o_0,a_0,\ldots,o_t)$ denotes the interaction history. The sandbox executes the command and returns an observation:
\begin{equation}
o_{t+1}=\operatorname{Exec}_p(a_t).
\end{equation}
The observation may contain file contents, standard output, execution failures, parsing errors, or evaluator diagnostics. The trajectory is written as
\begin{equation}
\tau=(o_0,a_0,o_1,a_1,\ldots,o_T).
\end{equation}

The final plan is parsed from \texttt{outputs/final\_plan.json}. UrbanSandbox then checks whether the plan satisfies the aggregate constraint function $\Psi_p(P,\mathcal{G}_p)$ and evaluates its planning score:
\begin{equation}
\operatorname{Eval}_p(P)=
\begin{cases}
S_p(P), & \Psi_p(P,\mathcal{G}_p)=1,\\
\operatorname{Error}_p(P), & \Psi_p(P,\mathcal{G}_p)=0.
\end{cases}
\end{equation}
Thus, plan validity and quality are determined by executable verification rather than language check. 

\begin{figure}[tbp]
    \centering
    \includegraphics[width=\linewidth]{figures/ATRL.pdf}
    \caption{Atomic-task reinforcement learning for executable urban planning. CityPlanner decomposes long-horizon sandbox planning into BuildPlan and ImprovePlan, and composes the two learned skills into iterative refinement at inference time.}
    \label{fig:atr}
\end{figure}

\subsection{Atomic-Task Reinforcement Learning}
\label{subsec:atomic_learning}
A pretrained language model provides useful priors for file inspection, structured generation, script writing, and tool use, but it is not by itself a reliable planner under hard spatial constraints. As shown in Figure~\ref{fig:atr}, directly training on complete sandbox trajectories requires assigning a sparse final reward to many preceding steps, such as state reading, plan construction, revision, and evaluation. These long and noisy trajectories make credit assignment difficult. CityPlanner therefore decomposes training into two atomic tasks, following the common structure of strong heuristic solvers: first construct an initial solution and then improve it by search. BuildPlan learns the construction stage from task files, while ImprovePlan learns the improvement stage from the incumbent plan and evaluator diagnostics. Each task has a shorter horizon and an independent task-level reward.

We use $\operatorname{Rollout}_{\pi_\theta}^{z}(\cdot)$ to denote a bounded multi-turn interaction between the policy and UrbanSandbox under atomic task $z$, whose output is the final plan submitted to \texttt{outputs/final\_plan.json}.

\paragraph{BuildPlan.}
BuildPlan is the construction task. Given the sandbox environment $\mathcal{E}_p$, which contains the city graph $\mathcal{G}_p$, candidate set $\mathcal{C}_p$, task constraints, and output interface, the policy generates an initial plan through a bounded sandbox rollout:
\begin{equation}
P_0=\operatorname{Rollout}_{\pi_\theta}^{\mathrm{build}}(\mathcal{E}_p).
\end{equation}
This task trains the model to construct a feasible executable plan from scratch.

\paragraph{ImprovePlan.}
ImprovePlan is the revision task. Given the sandbox environment $\mathcal{E}_p$, the current plan $P_t$, and evaluator diagnostics $\mathbf{d}_t$, the policy generates a revised plan:
\begin{equation}
\tilde{P}_{t+1}
=
\operatorname{Rollout}_{\pi_\theta}^{\mathrm{imp}}
(\mathcal{E}_p,P_t,\mathbf{d}_t),
\end{equation}
where $\mathbf{d}_t$ denotes the constraint and score feedback returned by UrbanSandbox. This task trains the model to improve an existing plan from feedback.

\paragraph{Reward.}
Both atomic tasks use the same plan-level terminal reward. Given a submitted plan $P$, the reward is its planning score if it satisfies the task constraints, and a failure penalty otherwise:
\begin{equation}
R_p(P)=
\begin{cases}
S_p(P), & \Psi_p(P,\mathcal{G}_p)=1,\\
R_{\mathrm{fail}}, & \text{otherwise}.
\end{cases}
\end{equation}

\paragraph{Learning Algorithm.}
We optimize the policy with GRPO~\cite{grpo} by sampling rollouts from BuildPlan and ImprovePlan. Each rollout receives the corresponding task-level reward. This trains the policy on bounded atomic skills, avoiding direct optimization over long and noisy trajectories.



\subsection{Iterative Inference}
\label{subsec:inference}
At inference time, CityPlanner composes the two learned atomic skills into an iterative planning procedure, as shown in Figure~\ref{fig:atr}. Given a test environment $\mathcal{E}_p$, CityPlanner first invokes BuildPlan to generate an initial plan $P_0$. UrbanSandbox evaluates this plan and returns its score and diagnostic feedback $\mathbf{d}_0$.
CityPlanner then repeatedly invokes ImprovePlan. At iteration $t$, the current best plan $P_t$ and diagnostics $\mathbf{d}_t$ are provided through the sandbox, and the model proposes a revised plan $\tilde{P}_{t+1}$. The proposal is then evaluated by UrbanSandbox before being accepted or rejected.

After each ImprovePlan call, UrbanSandbox evaluates the proposed plan. We accept a proposal only if it is better under a validity-first order: feasible plans are preferred to infeasible ones, and among feasible plans, higher scores are preferred. Denote this order by $\succ_p$. The update rule is
\begin{equation}
P_{t+1}=
\begin{cases}
\tilde{P}_{t+1}, & \tilde{P}_{t+1}\succ_p P_t,\\
P_t, & \text{otherwise}.
\end{cases}
\end{equation}
The loop stops after a fixed iteration budget or a patience budget, and returns the best-so-far plan.



==> 4-exp-bp.tex <==
\begin{table}[t]
\centering
\caption{UrbanSandbox dataset statistics across five urban clusters.}
\label{tab:urban_clusters}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lcc}
\toprule
\textbf{Region} & \textbf{Tiles} & \textbf{Representative Cities} \\
\midrule
Beijing--Tianjin--Hebei & 25,269 & Beijing, Tianjin, Shijiazhuang \\
Yangtze River Delta & 21,872 & Shanghai, Nanjing, Hangzhou \\
Chengdu--Chongqing & 19,266 & Chengdu, Chongqing, Mianyang \\
Mid--Yangtze & 19,488 & Wuhan, Yichang, Changsha \\
Pearl River Delta & 17,203 & Guangzhou, Shenzhen, Hong Kong \\
\bottomrule
\end{tabular}
}
\end{table}

\section{Experiments}
\label{sec:exp}

% We conduct experiments to evaluate CityPlanner on heterogeneous executable urban planning tasks. 
% The experiments are organized around four research questions:

% \begin{itemize}[leftmargin=*]
%     \item \textbf{RQ1: Overall effectiveness.} Can CityPlanner produce feasible and high-quality plans across different urban planning tasks and difficulty levels?
%     \item \textbf{RQ2: Test-time planning scaffold.} Can the UrbanSandbox-based workflow improve a frozen LLM planner without post-training?
%     \item \textbf{RQ3: Training and deployment contribution.} How much do SFT, GRPO, atomic-task RL, and iterative refinement deployment contribute?
%     \item \textbf{RQ4: Efficiency and refinement behavior.} Does CityPlanner improve planning quality with controlled interaction cost?
% \end{itemize}

\begin{table*}[t]
\centering
\caption{Performance comparison across tasks and difficulty levels. Results are reported as mean$\pm$std. The best result in each column is highlighted in bold, and the second-best result is underlined.}
\label{tab:overall_difficulty_std}
\scriptsize
\setlength{\tabcolsep}{2.5pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccc}
\toprule
\multirow{2}{*}{\textbf{Method}}
& \multicolumn{3}{c}{\textbf{Land Allocation}}
& \multicolumn{3}{c}{\textbf{Road Construction}}
& \multicolumn{3}{c}{\textbf{Station Placement}} \\
\cmidrule(lr){2-4}
\cmidrule(lr){5-7}
\cmidrule(lr){8-10}
& \textbf{Small} & \textbf{Medium} & \textbf{Large}
& \textbf{Small} & \textbf{Medium} & \textbf{Large}
& \textbf{Small} & \textbf{Medium} & \textbf{Large} \\
\midrule

\multicolumn{10}{l}{\textit{\textbf{Heuristic Methods}}} \\
\addlinespace[1pt]
GRASP
& 0.391$\pm$0.042
& 0.448$\pm$0.058
& 0.441$\pm$0.034
& \textbf{0.717$\pm$0.011}
& \underline{0.729$\pm$0.019}
& \underline{0.690$\pm$0.018}
& 0.279$\pm$0.024
& 0.064$\pm$0.009
& 0.020$\pm$0.001 \\

SA
& 0.395$\pm$0.086
& 0.441$\pm$0.097
& 0.431$\pm$0.044
& \underline{0.662$\pm$0.056}
& 0.567$\pm$0.065
& 0.596$\pm$0.074
& \underline{0.610$\pm$0.052}
& 0.437$\pm$0.094
& 0.353$\pm$0.078 \\

ALNS
& \underline{0.396$\pm$0.091}
& \underline{0.456$\pm$0.096}
& \underline{0.451$\pm$0.073}
& 0.653$\pm$0.063
& 0.513$\pm$0.059
& 0.510$\pm$0.077
& 0.501$\pm$0.073
& 0.434$\pm$0.080
& \underline{0.392$\pm$0.075} \\

\midrule
\multicolumn{10}{l}{\textit{\textbf{TSRL Methods}}} \\
\addlinespace[1pt]
MLP+PPO
& 0.205$\pm$0.015
& 0.276$\pm$0.011
& 0.271$\pm$0.014
& 0.070$\pm$0.066
& 0.166$\pm$0.069
& 0.135$\pm$0.049
& 0.222$\pm$0.021
& 0.132$\pm$0.011
& 0.153$\pm$0.018 \\

AM+PPO
& 0.184$\pm$0.014
& 0.248$\pm$0.011
& 0.248$\pm$0.010
& 0.269$\pm$0.032
& 0.256$\pm$0.025
& 0.307$\pm$0.010
& 0.224$\pm$0.017
& 0.175$\pm$0.026
& 0.194$\pm$0.011 \\

GNN+PPO
& 0.212$\pm$0.016
& 0.289$\pm$0.010
& 0.280$\pm$0.012
& 0.174$\pm$0.064
& 0.147$\pm$0.069
& 0.168$\pm$0.045
& 0.185$\pm$0.017
& 0.121$\pm$0.049
& 0.118$\pm$0.055 \\

\midrule
\multicolumn{10}{l}{\textit{\textbf{LLM Agents}}} \\
\addlinespace[1pt]
Qwen3.5
& 0.366$\pm$0.061
& 0.329$\pm$0.093
& 0.370$\pm$0.090
& 0.332$\pm$0.049
& 0.498$\pm$0.044
& 0.478$\pm$0.045
& 0.503$\pm$0.032
& 0.396$\pm$0.046
& 0.379$\pm$0.061 \\

Mimo V2.5
& 0.335$\pm$0.072
& 0.317$\pm$0.081
& 0.344$\pm$0.096
& 0.414$\pm$0.042
& 0.485$\pm$0.037
& 0.419$\pm$0.015
& 0.415$\pm$0.021
& 0.339$\pm$0.058
& 0.326$\pm$0.073 \\

DS-V4
& 0.323$\pm$0.095
& 0.364$\pm$0.083
& 0.360$\pm$0.056
& 0.334$\pm$0.035
& 0.579$\pm$0.038
& 0.527$\pm$0.039
& 0.527$\pm$0.021
& \underline{0.444$\pm$0.058}
& 0.381$\pm$0.052 \\

CityPlanner
& \textbf{0.402$\pm$0.014}
& \textbf{0.459$\pm$0.031}
& \textbf{0.451$\pm$0.026}
& 0.609$\pm$0.021
& \textbf{0.735$\pm$0.014}
& \textbf{0.704$\pm$0.054}
& \textbf{0.612$\pm$0.060}
& \textbf{0.462$\pm$0.034}
& \textbf{0.397$\pm$0.062} \\

\bottomrule
\end{tabular}
}
\end{table*}

\subsection{Experimental Setup}
\label{subsec:exp_setup}
\paragraph{Benchmark.}
We construct the benchmark from large-scale OpenStreetMap data over diverse urban regions in China, with details of data collection and preprocessing provided in Appendix~\ref{app:dataset_details}. The benchmark contains 5,670 planning instances over 1,890 urban tiles across three tasks. All tasks are evaluated through UrbanSandbox, where each method must generate an executable plan and obtain its final score from the task evaluator.

\paragraph{Baselines.}
We compare CityPlanner with three groups of baselines: \textbf{heuristic methods}, including GRASP, SA, and ALNS; \textbf{task-specific reinforcement learning methods}, including MLP+PPO, AM+PPO, and GNN+PPO; and \textbf{general LLM agents}, including Qwen3.5, Mimo V2.5, and DS-V4, which solve the tasks through UrbanSandbox without task-specific training. CityPlanner is based on Qwen3-8B and is post-trained in two stages: we first adapt the model to a Terminal-Bench-style interaction format using the public OpenThoughts SFT data, and then train it with atomic-task RL on our UrbanSandbox tasks. Implementation details of all methods are provided in Appendix~\ref{app:implementation}.

\paragraph{Evaluation protocol.}
All methods are evaluated on the same instances. Agent-based methods use the same sandbox files, output format, and interaction budget. In the main comparison, we use the task-specific objective score returned by the evaluator as the primary metric. The score definitions follow the original task objectives and are detailed in Appendix~\ref{app:task_definitions}. For all tasks, higher scores indicate better planning quality. Each method is evaluated three times with different random seeds, and we report the mean and standard deviation.

\subsection{Overall Performance}
\label{subsec:overall_performance}
Table~\ref{tab:overall_difficulty_std} reports the main comparison across three tasks and three difficulty levels. We summarize the results as follows.

\noindent~$\bullet$ \emph{CityPlanner achieves the strongest overall performance.}
CityPlanner obtains the best score in 8 out of 9 settings. This indicates that CityPlanner is consistently effective across heterogeneous planning tasks and scales.

\noindent~$\bullet$ \emph{Strong heuristics remain competitive baselines.}
Among non-agent baselines, heuristic methods generally perform best. For example, GRASP achieves the best score on small Road Construction and remains the second-best method on medium and large Road Construction. SA is also highly competitive on small Station Placement. These results show that search heuristics are still strong, especially on smaller or more regular instances.

\noindent~$\bullet$ \emph{Task-specific RL methods are less effective under limited data.}
The TSRL baselines perform substantially worse across all tasks. 
This suggests that, under limited training data, task-specific neural policies fail to learn effective planning strategies for these executable urban planning tasks.



\noindent~$\bullet$ \emph{Agent-based methods are competitive on complex settings.}
General LLM agents achieve competitive results in several larger settings, suggesting that tool use and iterative reasoning are useful for complex planning tasks. CityPlanner further strengthens this trend by combining executable feedback with atomic-task training and iterative refinement. These results indicate that agent-based planning becomes more effective as the candidate space grows and direct search becomes harder.





\subsection{Effect of Test-Time Planning Scaffold}
\label{subsec:scaffold_effect}

% Put Table~\ref{tab:deepseek_scaffold} here.
\begin{table}[t]
\centering
\caption{Comparison of test-time planning strategies using DeepSeek as a frozen planner. 
Ours (Scaffold) denotes our UrbanSandbox-based atomic workflow without post-training.}
\label{tab:deepseek_scaffold}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{\textbf{Method}}
& \multicolumn{2}{c}{\textbf{Land Allocation}}
& \multicolumn{2}{c}{\textbf{Road Construction}}
& \multicolumn{2}{c}{\textbf{Station Placement}} \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}
& \textbf{Feas.}$\uparrow$ & \textbf{Score}$\uparrow$
& \textbf{Feas.}$\uparrow$ & \textbf{Score}$\uparrow$
& \textbf{Feas.}$\uparrow$ & \textbf{Score}$\uparrow$ \\
\midrule
Text-only
& 22.20\% & 0.0670
& 27.77\% & 0.0460
& 17.19\% & 0.0630 \\

EoH
& 87.80\% & 0.3052
& 21.00\% & 0.0860
& \underline{97.80\%} & \underline{0.2460} \\

FunSearch
& \underline{91.10\%} & \underline{0.3232}
& \underline{32.00\%} & \underline{0.1537}
& 81.10\% & 0.1456 \\

\midrule
Ours
& \textbf{95.69\%} & \textbf{0.3490}
& \textbf{100.00\%} & \textbf{0.4780}
& \textbf{98.15\%} & \textbf{0.4530} \\
\bottomrule
\end{tabular}
}
\end{table}

\begin{table}[t]
\centering
\caption{Ablation under the full UrbanSandbox environment. 
ATRL denotes atomic-task RL, and CityPlanner further applies iterative refinement deployment.}
\label{tab:training_deployment_ablation}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{\textbf{Method}}
& \multicolumn{2}{c}{\textbf{Land Allocation}}
& \multicolumn{2}{c}{\textbf{Road Construction}}
& \multicolumn{2}{c}{\textbf{Station Placement}} \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}
& \textbf{Feas.}$\uparrow$ & \textbf{Obj.}$\uparrow$
& \textbf{Feas.}$\uparrow$ & \textbf{Obj.}$\uparrow$
& \textbf{Feas.}$\uparrow$ & \textbf{Obj.}$\uparrow$ \\
\midrule
Qwen3-8B
& 15.29\% & 0.1067
& 21.95\% & 0.1290
& 23.31\% & 0.1020 \\

\quad + SFT
& 82.40\% & 0.3120
& 87.10\% & 0.3077
& 82.40\% & 0.3120 \\

\quad + GRPO
& \underline{89.60\%} & 0.3440
& \underline{94.20\%} & 0.5860
& \underline{91.30\%} & 0.3790 \\

\quad + ATRL
& \textbf{100.00\%} & \underline{0.4210}
& \textbf{100.00\%} & \underline{0.6820}
& \textbf{100.00\%} & \underline{0.4670} \\

\midrule
CityPlanner
& \textbf{100.00\%} & \underline{0.4374}
& \textbf{100.00\%} & \underline{0.7163}
& \textbf{100.00\%} & \underline{0.4945} \\

\quad+ Qwen14B
& \textbf{100.00\%} & \textbf{0.4498}
& \textbf{100.00\%} & \textbf{0.7312}
& \textbf{100.00\%} & \textbf{0.5116} \\
\bottomrule
\end{tabular}
}
\end{table}


\subsection{Ablation Study}
\label{subsec:ablation}

To further verify the effectiveness of our design, we conduct ablation studies from two aspects: the test-time planning scaffold and the atomic-task training strategy. The first study isolates the effect of UrbanSandbox-based executable planning without any post-training. The second study examines how supervised fine-tuning, GRPO, atomic-task RL, and iterative deployment contribute to the final CityPlanner performance.

\paragraph{Effect of UrbanSandbox.}
We first evaluate whether the proposed planning scaffold itself is useful for a frozen LLM planner. In this experiment, all methods use DeepSeek as the frozen planner, and no task-specific post-training is applied. 
We compare four test-time strategies. \textbf{Text-only prompting} allows the frozen LLM to perform multi-turn reasoning, but it cannot call tools or execute the evaluator; the final plan is generated purely from textual reasoning. \textbf{EoH} and \textbf{FunSearch} are LLM-guided heuristic search frameworks. We adapt them by asking the frozen LLM to generate and iteratively refine executable heuristic programs, which are evaluated by the task evaluator and selected according to their scores. \textbf{Ours} uses the proposed UrbanSandbox-based atomic workflow, where the frozen LLM can inspect task files, execute commands, evaluate candidate plans, and revise its output, but no model parameters are updated.

Table~\ref{tab:deepseek_scaffold} reports the results. Text-only prompting performs poorly, with feasibility below 30\% on all three tasks, indicating that direct generation is insufficient for constrained urban planning. EoH and FunSearch improve performance on some tasks but remain unstable; for example, their Road Planning feasibility is only 21.00\% and 32.00\%, respectively. In contrast, our scaffold achieves the best feasibility and score on all tasks. These results show that executable file inspection, evaluator feedback, and structured plan revision make test-time planning substantially more reliable even without updating the LLM.

\paragraph{Effect of atomic-task training.}
We then evaluate the contribution of training and deployment components under the full UrbanSandbox environment. All variants share the same experimental setting unless otherwise specified. We compare six variants: \textbf{Qwen3-8B}, the raw instruction model without post-training; \textbf{+SFT}, which applies supervised fine-tuning on sandbox planning trajectories; \textbf{+GRPO}, which further optimizes the model with standard flat RL; \textbf{+ATRL}, which replaces trajectory-level training with atomic-task RL over BuildPlan and ImprovePlan; \textbf{CityPlanner}, which further applies iterative refinement at inference time; and \textbf{+Qwen14B}, which replaces the 8B base model with Qwen3-14B while keeping the same CityPlanner pipeline.

Table~\ref{tab:training_deployment_ablation} reports the results. The raw model rarely produces feasible plans, with feasibility below 25\% on all tasks, showing that instruction-following ability alone is insufficient for executable urban planning. SFT improves feasibility to over 80\%, and GRPO further improves objective scores. ATRL brings the largest feasibility gain, improving feasibility over GRPO by an average of 8.3 percentage points and reaching 100.00\% feasibility on all three tasks. It also improves objective scores over GRPO by 20.7\% on average. CityPlanner further improves objective scores through iterative refinement, achieving an average relative gain of 4.9\% over ATRL. Replacing the base model with Qwen3-14B brings an additional average gain of 2.8\%, indicating that the proposed training and deployment pipeline can also benefit from larger base models. Overall, these results verify the effectiveness of each component.




\begin{figure}[t]
    \centering
    % \begin{subfigure}{\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/quality_time_bubble.png}
    % \caption{Quality--time trade-off.}
    \label{fig:quality_time_bubble}
    % \end{subfigure}
    
    % \vspace{0.5em}
    
    % \begin{subfigure}{\linewidth}
    %     \centering
    %     \includegraphics[width=\linewidth]{figures/avg_turn.png}
    %     \caption{Average interaction turns of LLM agents.}
    %     \label{fig:avg_turn}
    % \end{subfigure}
    
    \caption{Efficiency analysis of CityPlanner and competing methods. }
    % (a) compares the quality--time trade-off averaged over tasks, where CityPlanner achieves the best overall quality rank with moderate runtime. 
    % (b) reports the average number of interaction turns under different task difficulties, showing that CityPlanner uses a comparable number of turns to other strong LLM agents while maintaining stronger planning quality.}
    \label{fig:efficiency_analysis}
\end{figure}

% Put Figure~\ref{fig:best_curve_road} here.
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/best_curve_road.png}
    \caption{Best-so-far refinement curve on a representative road construction instance.}
    \label{fig:best_curve_road}
\end{figure}


\subsection{Efficiency and Refinement Behavior}
\label{subsec:efficiency_refinement}

We further evaluate CityPlanner from the efficiency perspective. The analysis focuses on two aspects: the quality--time trade-off across different planning paradigms, and the refinement behavior of CityPlanner during iterative deployment.

\paragraph{Quality--time trade-off.}
Figure~\ref{fig:efficiency_analysis} compares different methods by their average planning quality and runtime. The results show clear differences among planning paradigms. TSRL methods are the fastest because they only require lightweight policy inference, but they obtain low solution quality. Heuristic methods achieve competitive quality on some tasks, but require non-trivial search time. LLM agents are generally slower due to multi-turn reasoning and sandbox interaction. CityPlanner achieves the best overall planning quality with moderate runtime, showing a favorable quality--time trade-off compared with both generic LLM agents and search-based methods.

\paragraph{Refinement behavior.}
Figure~\ref{fig:best_curve_road} shows the best-so-far score during a representative road construction episode. The curve illustrates how CityPlanner improves the solution through iterative refinement. DeepSeek stays in a low-score region, suggesting that direct long-horizon planning struggles to recover from invalid or non-improving submissions. In contrast, CityPlanner quickly obtains a valid intermediate plan and continues to improve it using evaluator feedback. Its best-so-far score first surpasses ALNS and SA, and eventually exceeds the Greedy baseline after additional refinement steps. These results show that iterative deployment enables stable plan improvement instead of repeatedly regenerating solutions from scratch.

